Linear Algebraic Structure of Word Senses, with Applications to Polysemy

Word embeddings are ubiquitous in NLP and information retrieval, but it is unclear what they represent when the word is polysemous. Here it is shown that multiple word senses reside in linear superposition within the word embedding and simple sparse coding can recover vectors that approximately capture the senses. The success of our approach, which applies to several embedding methods, is mathematically explained using a variant of the random walk on discourses model (Arora et al., 2016). A novel aspect of our technique is that each extracted word sense is accompanied by one of about 2000 "discourse atoms" that gives a succinct description of which other words co-occur with that word sense. Discourse atoms can be of independent interest, and make the method potentially more useful. Empirical tests are used to verify and support the theory.

==> explanation.tex <==
 \section{Explanation of Main Claim}
   \label{sec:explanation}
	
We now prove the Main Claim from Section~\ref{subsec:explanation},  using notations and simplifications introduced there. Throughout this section, it is assumed that the norm of the word vectors is upper bounded by a small constant (say $5$) and the dimension $d$ is much bigger, say $300$. Thus the ratio of the norm of a word vector and $d$ is considered \textquotedblleft tiny\textquotedblright. We also denote $v_1 = v_{w_1}$ and $v_2 = v_{w_2}$. Sets $T_1, T_2$ were introduced earlier, and $\kappa_1, \kappa_2$ were defined in the Main Claim. 

Let's simplify objective $f(z)$ in (\ref{eqn:zopt}).
%Recall the definition of sets $T_1$ and $T_2$ in Section~\ref{subsec:explanation}.
 By Simplification 2, for $i \in \{1,2\}$ and $\chi\in T_i$, we have $\displaystyle p(\chi,w) = p(\chi,w_i)$, so 
\small
\begin{align}
\pmi(\chi,w) & = \log \frac{p(\chi, w)}{p(\chi)p(w)} = \frac{p(\chi,w_i)}{p(\chi)(p(w_1)+p(w_2))} \nonumber\\
& =\pmi(\chi,w_i) - \log\left(\frac{p(w_1)+p(w_2)}{p(w_i)}\right) \nonumber\\
& =\pmi(\chi,w_i) -\kappa_i  ~\textup{for}~\chi \in T_i. \label{eqn:sim2}
\end{align}
%\Tnote{It's not immediate clear how this is obtained and we should recall the definition of %$\kappa$}\normalsize
Furthermore, Simplification 1 implies
$
\pmi(\chi, w_i) = \inner{v_{\chi},w_i}, ~\textup{for}~\chi \in T_i. 
$
\normalsize
Then $f(z)$ is simplified by \eqref{eqn:sim2}  as
\small
\begin{align*}
  f(z) =  \sum_{i=1,2}~\underbrace{\sum_{\chi\in T_i} p(\chi, w_i) (\inner{v_\chi, v_i - z}- \kappa_i)^2}_{f_i(z)} 
\end{align*}
\normalsize
Clearly, if shifts $\kappa_1$ and $\kappa_2$ were zero, then $f_1$ and $f_2$ would be minimized at $z = v_1$ and $z = v_2$ respectively by definition. Intuitively, our argument will consist of two parts. First, we show that even with the non-zero constant shift $\kappa_1$ and $\kappa_2$:
\begin{align}
&   \textup{argmin } f_i(z)= (1-\kappa_i c_i)v_i, \label{eqn:minimizer}
\end{align}
\normalsize
where $c_1$ and $c_2$ are small constants to be determined later. 
That is, the minimizers of $f_1$ and $f_2$ are only changed by a scaling due to the presence of the constant shift $\kappa_1$ and $\kappa_2$. Second, we will show 
\small
\begin{align}
  \textup{argmin } f(z) \approx \textup{argmin } f_1(z) + \textup{argmin } f_2(z). \label{eqn:additivity}
\end{align}
\normalsize
From~\eqref{eqn:minimizer} and~\eqref{eqn:additivity}, the claim follows. 

We prove (\ref{eqn:minimizer}) for $f_1$; leaving $f_2$ as analogous.
To analyze the structure of $f_1$, denote the mean of the vectors of words that co-occur with $w_1$ as $\mu_1 = \sum_{\chi} p(\chi, w_1) v_\chi$, and denote their second moment as $\Sigma_1 = \sum_{\chi} p(\chi, w_1) v_\chi v_\chi^\top$. (Define $\Sigma_2,\mu_2$ similarly for word $w_2$). Then
\small
\begin{align*}
	f_1(z) = & ~(v_1-z)^{\top}\Sigma_1(v_1-z)  -2 \kappa_1 \mu_1^{\top} (v_1-z) + C
\end{align*}
\normalsize
where $C$ is a constant independent of $z$. Simplification 3 lets us gets a handle on $f_1(z)$. 

%\noindent{\textbf{Simplification 3}:} \emph{For} $i \in \{1,2\}, \mu_i$ \emph{has the form} $b_i v_{w_i}$ \emph{, and} $\Sigma_i$ \emph{has the form} $\gamma_i v_{w_i} v_{w_i}^\top + \tau_i I,$ \emph{where} $b_i, \gamma_i$ \emph{,and} $\tau_i$ \emph{are scalar parameters.}


\noindent{\textbf{Simplification 3}:} % \emph{For} $i \in \{1,2\}, \mu_i$ 
$\mu_1$ \emph{has the form} $b_1 v_{1}$ \emph{, and} $\Sigma_1$ \emph{has the form} $\gamma_1 v_{1} v_{1}^\top + \tau_1 I,$ \emph{where} $b_1, \gamma_1$ \emph{,and} $\tau_1$ \emph{are scalar parameters and $\tau_1$ is tiny.}. We assume similar structure for $\mu_2$ and $\Sigma_2$ (with $b_2,\gamma_2,\tau_2$ defined similarly). 

%\Tnote{Tried to avoid using index $i$. }

\noindent {\em Justification of Simplification 3.}~ \newcite{randomdiscourses} shows evidence (contrary to intuition) that word vectors are distributed fairly uniformly in space, and in the bulk have many properties similar to random vectors. Since words that co-occur with $w_1$ have (by the PMI model) nontrivial inner product with $v_1$,  the word vectors in $T_1$ ought to behave roughly like $\rho v_1 + \xi$ \emph{where} $\rho$ \emph{is a scalar and }$\xi$ \emph{is a spherical Gaussian vector with comparable norm to that of} $\rho v_1$. 
Since word vectors have norm $O(1)$, it is reasonable to assume $\mathbb{E}[\rho]$ 
and $| \mathbb{E} [v_\chi]|_2$ are both at most $O(1)$ and so Simplification 3 for $T_1$ then follows, with $\tau_1$ roughly $O(1)/d$, which is tiny. 
%\hfill $\qedsymbol$

Having justif{i}ed Simpli{f}ication 3 we return to the argument for the main claim. 
The quadratic form $\Sigma_1$ can be better understood after picking an orthogonal basis in which it is diagonalized. 
Since $w_1$ and $w_2$ are a pair of words randomly chosen, one expects their PMI to be 0, and thus by Simplification~1, $v_1^\top v_2 = 0$. So define %\yingyu{added the definition for $R$}
$R$ be the linear transformation defined as $
 R = [v_1/ \|v_1\|^2, v_2 / \|v_2\|^2, u_3, \cdots, u_d]^\top
$ 
where $u_3,\cdots, u_d$ are an arbitrary set of basis vectors for the complement of the subspace spanned by $v_1$ and $v_2$.  
Then we have $R$ diagonalize the covariance matrix 
since $\displaystyle \Lambda = R^{-\top}\Sigma_1R^{-1} = \textup{diag}(\tilde{\gamma}_1, \tilde{\tau}_1,\tau_1,\dots, \tau_1)$ is a diagonal matrix, with $\tilde{\gamma}_1 = \gamma_1 \|v_1\|^4 + \tau_1\|v_1\|^2$ and $\tilde{\tau}_1 = \tau_1 \|v_1\|^2$. Moreover, we have $R v_1 = e_1$, $R v_2 = e_2$. After this diagonalization, letting $\tilde{z} = Rz$,  
\small
\begin{align}
	f_1(z) = & ~ (e_1-\tilde{z})^T \Lambda(e_1-\tilde{z}) + 2\kappa_1 b_1 e_1^T (e_1-\tilde{z}) + C \nonumber\\
	= & ~ \tilde\gamma_1(1- \tilde{z}_1)^2 - 2\kappa_1 b_1(1-\tilde{z}_1) \nonumber\\
	& ~ + \tilde\tau_1 \tilde{z}_2^2 +  \tau_1 \sum_{j\neq 1,2} \tilde{z}_j^2 + C. 
 \label{eqn:f1_diag}
\end{align}
\normalsize
Let $z^{\star}$ denote the minimizer of $f_1$. Thus we have $\tilde{z}^{\star}_j  = 0$ for $j\neq 1$, and $\tilde{z}^{\star}_1$ is the minimizer of the univariate quadratic function $\tilde\gamma_1(1- \tilde{z}_1)^2 - 2\kappa_1 b_1(1-\tilde{z}_1)$. By elementary calculation we get $\tilde{z}^{\star}_1 = 1- c_1\kappa_1$ with $c_1 = b_1/\tilde\gamma_1$. Therefore, we have $\tilde{z}^{\star} = (1-c_1\kappa_1)e_1$. 
Since $\tilde{z} = Rz$, the minimizer of $f_1(z)$ is 
\small 
\begin{align*}
  \textup{argmin}~f_1(z) = R^{-1}\tilde{z}^{\star} = (1-c_1 \kappa_1)v_1.
\end{align*}
\normalsize

Having proved equation~\eqref{eqn:minimizer}, we turn to~\eqref{eqn:additivity}. The additive structure of \eqref{eqn:additivity} is obviously false in general, but holds here because $f_1$ and $f_2$ interact with each other in a rather limited way. As we have shown, $f_1(z)$ is only sensitive to the projection of $z$ on $v_1$, and $f_2$ only to the projection of $z$ on $v_2$. Hence the minimizer of $f_1+f_2$ is achieved when $z$ has the right projection to both $v_1$ and $v_2$. Formally, repeating the argument above, we have an  expression similar for $f_2$ to (\ref{eqn:f1_diag}). Then
\small 
\begin{align}
  f(z) = & ~ f_1(z) + f_2(z) \nonumber\\
   = & ~ \tilde\gamma_1(1- \tilde{z}_1)^2 - 2\kappa_1 b_1(1-\tilde{z}_1) + \tilde\tau_2 \tilde{z}_1^2 \tag{line 1} \label{line1}\\
	 +&  \tilde\gamma_2(1- \tilde{z}_2)^2 - 2\kappa_2 b_2 (1-\tilde{z}_2) + \tilde\tau_1 \tilde{z}_2^2 \tag{line 2}\label{line2}\\
	+& (\tau_1 + \tau_2) \sum_{j\neq 1,2} \tilde{z}_j^2 + C'. \label{eqn:50}
	\end{align}
\normalsize
%\Tnote{defined $\tilde{z}^{\star\star}$ so that it won't get confused with previous $\tilde{z}^{\star}$}
%
Let $\tilde{z}^{\star\star}$ be the optimum of RHS of~\eqref{eqn:50}. Then $\tilde{z}_j^{\star\star} = 0$ for $j \neq 1,2$, and $\tilde{z}^{\star\star}_1$ and $\tilde{z}^{\star\star}_2$ are the minimizers of~\eqref{line1} and~\eqref{line2}, respectively. Again, by elementary calculation, we can compute $z^{\star\star}$, and it translates to that the optimum of $f(z)$ is 
\small 
\begin{align*}
\textup{argmin } f(z) = R^{-1} \tilde{z}^{\star\star} = \frac{1 - c_1 \kappa_1}{1 + \epsilon_1} v_1 + \frac{1 - c_2 \kappa_2}{1 + \epsilon_2} v_2
\end{align*}
\normalsize
where $c_i = b_i/\tilde\gamma_i$, $\epsilon_1 = \tilde\tau_2/\tilde\gamma_1$, and $\epsilon_2 = \tilde\tau_1/\tilde\gamma_2$. 	

%Finally, we estimate the quantities $c_i$ and $\epsilon_i$ intuitively.  
%We have established that $v_w$ is a linear combination of $v_1$ and $v_2$, and that the coefficients depend on the logarithm of the frequency ratio. However, the experiment in Section~\ref{sec:linear} shows more: $\epsilon_i \ll 1$, and $c_i$ are in the order of 1. 


%\Tnote{Reorganized below}
Towards completing the proof of  the main claim, we now estimate $\epsilon_2$ and $c_1$ (similar arguments hold for $\epsilon_1$ and $c_2$). 
We fist estimate $\tilde{\gamma}_1$ and $b_1$. By the definition of $\Sigma_1$ and simplification 3, we have that $v_1^{\top}\left(\sum_{\chi\in T_1} p(\chi,w_1)v_\chi v_\chi^T\right)v_1=v_1^{\top}\Sigma_1 v_1 = \gamma_1 \|v_1\|^4 + \tau_1\|v_1\|^2$. Since $\tau_1\ll \gamma_1$, we have that $\tilde{\gamma_1}\approx \gamma_1$ and that
\vspace{-0.05in}
\small 
\begin{align} \label{eqn:gamma}
\gamma_1\approx \tilde\gamma_1 \approx \sum_{\chi\in T_1} p(\chi, w_1)\inner{v_\chi,v_1}^2/\|v_1\|^4,
\end{align}
\normalsize
and a similar expression for $\tilde\gamma_2$. 
Moreover, by Simplification 3, we have $b_1 \|v_1\|^2
 = \mu_1^\top v_1 = \sum_{\chi \in T_1} p(\chi,w)\inner{v_1,v_\chi} $ and therefore $b_1 = \frac{1}{\|v_1\|^2} \sum_{\chi \in T_1} p(\chi,w)\inner{v_1,v_\chi} $. Now we are ready to estimate $c_1$, %Plugging in the estimation for $\gamma_1$ in \eqref{eqn:gamma} we obtain 
\small 
\begin{align}
c_1  = b_1/\gamma_1 \approx \frac{ \sum_{\chi\in T_1} p(\chi,v_1)\|v_1\|^2\inner{v_\chi,v_1}}{\sum_{\chi\in T_1} p(\chi,v_1)\inner{v_\chi,v_1}^2}\,. \label{eqn:41}\end{align} 
\normalsize
Note that for every $\chi\in T_1$, we expect that corresponding terms in the sums in the numerator and denominator are within constant factor, that is, $\|v_1\|^2 \inner{v_{\chi},v_1} \asymp \inner{v_\chi, v_1}^2$. This again can be seen if the vectors in $T_1$ are thought of as $v_1+ \xi$, as in the justification of Simplification 3,  where $\xi$ is a random vector with similar norm as $v_1$. Thus we obtain that $c_1$ is on the order of 1. 
%Note that RHS of~\eqref{eqn:41} has both numerator and denominator being homogeneous polynomials of $\chi$ and $v_1$ with degree 4, therefore we expect the overall expression is on the order of 1. 

%$Therefore, $c_1$ is expected to be $O(1)$ since $\|v_1\|$ and $\inner{\chi,v_1}$ are all $O(1)$.   \yingyu{$\|v_1\|^2 \in [2, 8]$ in our experiments, so we can claim it is $O(1)$?}
%So $\gamma_1/\gamma_2 \ll d \|v_2\|^2$ translates roughly to $p(w_1)/p(w_2) \ll d \|v_2\|^2$, which is true for the experiment. %\Tnote{``I am not quit sure what this means''} \yingyu{It means that $p(w_1)/p(w_2) \ll d \|v_2\|^2$ is satisfied for the $w_1$ and $w_2$ used in our experiments in Section 2}

Finally, recall the estimates for $\tilde{\tau_1}$ and $\tilde{\gamma_2}$, we have  $\epsilon_2 = \tilde\tau_1/\tilde\gamma_2 = \tau_1/ (\gamma_2 \|v_2\|^2 + \tau_2)$.
As shown in the justification of Simplification 3, we have $\tau_1 \approx \gamma_1/d$ and it follows that $\epsilon_2 \lesssim \gamma_1/\gamma_2\cdot 1/d$.  From equation~\eqref{eqn:gamma} (and the corresponding expression for $\gamma_2$ we can see that $\gamma_1/\gamma_2$ stays on the order of 1 as $d$ goes to infinity. Therefore we have $\epsilon_2 \lesssim\gamma_1/\gamma_2\cdot 1/d\ll 1$,which completes the proof. %\ll d \|v_2\|^2$, which implies $\epsilon_2  \ll 1$.


==> figure/figure_sciences_atoms.tex <==


	\begin{figure*}[!ht]
		\begin{minipage}{\textwidth}
			\includegraphics[width=\columnwidth]{figures-meta-atom/scientific_meta_atoms}
		\end{minipage}
		
		\begin{minipage}{\textwidth}
			\centering
			{\small
			\begin{tabular}{|l|l|l|l|l|l|}
				\hline Atom & 28 & 2016& 468 & 1318 & 411 \\
				\hline
				& logic & graph & boson & polyester & acids\\
				& deductive& subgraph & massless& polypropylene & amino\\
				& propositional & bipartite& particle & resins & biosynthesis\\
				& semantics& vertex& higgs & epoxy & peptide \\
				\hline
				tag & {\em logic} & {\em graph theory} & {\em particle physics} & {\em polymer} & {\em biochemistry}\\
				\hline 
			\end{tabular}
			}
		\end{minipage}
		\medskip
		\caption{Some atoms of discourse (purple circles) related to scientific fields and their meta-atoms (yellow circles) found by the second level sparse coding.  The connecting line corresponds to discourse atoms that use the meta atoms in the coding. Thus the atom for biochemistry is found to be expressed using a linear combination of the meta discourse vector of chemistry and biology (plus noise).}
		%\caption{Scientific atoms found and their meta-atoms: We found meta discourses of math, physics, chemistry and biology. The figure above shows the atoms that uses them: e.g., discourse vector of biochemistry is approximately a linear combination of the meta discourse vector of chemistry and biology (plus noise), while the number theory discourse vector is approximately the math meta discourse vector plus noise. }
		\label{fig:metaatom_science} 
	\end{figure*}


==> figure/figure_sports_atoms.tex <==


	\begin{figure*}[!t]
		\begin{minipage}{\textwidth}
		\centering
			\includegraphics[width=0.95\columnwidth]{figures-meta-atom/sport_meta_atoms}
		\end{minipage}
		
\vspace{-1mm}

		\begin{minipage}{\textwidth}
			\centering
			{\small
			\begin{tabular}{|l|l|l|l|l|l|l|l|}
				\hline Atom & 722 & 407 & 1164 & 1623 & 114 & 1932 & 633 \\
				\hline
				&          helicopter &               sedan &           sportscar &                race &                giro &             skating &        cheerleading \\
&         helicopters &           hatchback &             drivers &             podiums &              vuelta &              skater &            softball \\
&            sikorsky &              sedans &          motorsport &               races &                 uci &             skaters &          volleyball \\
&            aircraft &             hardtop &              racing &                laps &                 ttt &                 isu &             frisbee \\
				\hline
				tag & {\em aircraft } & {\em car model} & {\em sports car} & {\em  general racing} & {\em bike racing} &     {\em skating  }  &      {\em sports type } \\
				\hline 
			\end{tabular}
			}
		\end{minipage}
		
		%\caption{Meta-atoms for transportation, racing, and sports. The figure shows the atoms that uses them, where atoms/meta-atoms are tagged manually. The table shows the top 4 nearest words and tags for some atoms.}
		%\label{fig:sportmetaatom} 
		\caption{ Meta-atoms for transportation, racing, and sports. The figure shows the atoms that uses them, where atoms/meta-atoms are tagged manually. The table shows the top 4 nearest words and tags for some atoms.}
		\label{fig:metaatom_sports}
	\end{figure*}


==> figures-meta-atom/figure_food_atoms.tex <==


	\begin{figure*}[!t]	
		\begin{minipage}{\textwidth}
			\centering
			\includegraphics[width=0.82\columnwidth]{figures-meta-atom/food_meta_atoms}
		\end{minipage}
				
\vspace{-5mm}

		\begin{minipage}{\textwidth}
			\centering
			{\small
			\begin{tabular}{|l|l|l|l|l|l|l|l|}
				\hline Atom &6  & 1273 & 128 & 1549 & 959 &1109 & 1280\\
				\hline
&              cooked &               cakes &              drinks &              banana &              onions &            garlic &             grilled \\
&               fried &             dessert &               drink &             coconut &             cabbage &            spices &                beef \\
&                dish &                cake &            beverage &               beans &              garlic &               coriander &                pork \\
&              boiled &            pastries &           beverages &           sugarcane &             spinach &     sauce &              cooked \\
				\hline
				tag & {\em cooking } & {\em dessert} & {\em drinks} & {\em  fruit} & {\em vegetable} &     {\em spices}  &      {\em grill} \\
				\hline 
			\end{tabular}
			}
		\end{minipage}
		
		%\caption{Meta-atom for food. The figure shows the atoms that uses them, where atoms/meta-atoms are tagged manually. The table shows the top 4 nearest words and tags for some atoms.}
		%\label{fig:foodmetaatom} 
	\caption{Meta-atom for food. The figure shows the atoms that uses them, where atoms/meta-atoms are tagged manually. The table shows the top 4 nearest words and tags for some atoms.}
	\label{fig:metaatom_food}
	\end{figure*}


==> figures-meta-atom/figure_sciences_atoms.tex <==


	\begin{figure*}[!ht]
				\vspace{-5mm}
		%\begin{minipage}{\textwidth}
			\includegraphics[width=0.85\textwidth]{figures-meta-atom/scientific_meta_atoms}
		%\end{minipage}
		%\begin{minipage}{\textwidth}
			\centering
			{\small
			\begin{tabular}{|l|l|l|l|l|l|}
				\hline Atom & 28 & 2016& 468 & 1318 & 411 \\
				\hline
				& logic & graph & boson & polyester & acids\\
				& deductive& subgraph & massless& polypropylene & amino\\
				& propositional & bipartite& particle & resins & biosynthesis\\
				& semantics& vertex& higgs & epoxy & peptide \\
				\hline
				tag & {\em logic} & {\em graph theory} & {\em particle physics} & {\em polymer} & {\em biochemistry}\\
				\hline 
			\end{tabular}
			}
		\vspace{1mm}
		\caption{Some atoms of discourse (small circles) related to scientific fields and their meta atoms (large circles) found by the second level sparse coding.  The connecting line corresponds to discourse atoms that use the meta atoms in the coding. 
		Thus the atom {\em biochemistry} is found to be expressed approximately using a linear combination of the meta atoms {\em chemistry} and {\em biology}. 
		The tags are manually labeled, and the table shows the nearby words for some atoms with corresponding tags in the figure.}
		%\caption{Scientific atoms found and their meta-atoms: We found meta discourses of math, physics, chemistry and biology. The figure above shows the atoms that uses them: e.g., discourse vector of biochemistry is approximately a linear combination of the meta discourse vector of chemistry and biology (plus noise), while the number theory discourse vector is approximately the math meta discourse vector plus noise. }
		\label{fig:metaatom_sciences} 
		\vspace{-0.1in}
	\end{figure*}


==> figures-meta-atom/figure_sports_atoms.tex <==


	\begin{figure*}[!t]
		\begin{minipage}{\textwidth}
		\centering
			\includegraphics[width=0.95\columnwidth]{figures-meta-atom/sport_meta_atoms}
		\end{minipage}
		
\vspace{-1mm}

		\begin{minipage}{\textwidth}
			\centering
			{\small
			\begin{tabular}{|l|l|l|l|l|l|l|l|}
				\hline Atom & 722 & 407 & 1164 & 1623 & 114 & 1932 & 633 \\
				\hline
				&          helicopter &               sedan &           sportscar &                race &                giro &             skating &        cheerleading \\
&         helicopters &           hatchback &             drivers &             podiums &              vuelta &              skater &            softball \\
&            sikorsky &              sedans &          motorsport &               races &                 uci &             skaters &          volleyball \\
&            aircraft &             hardtop &              racing &                laps &                 ttt &                 isu &             frisbee \\
				\hline
				tag & {\em aircraft } & {\em car model} & {\em sports car} & {\em  general racing} & {\em bike racing} &     {\em skating  }  &      {\em sports type } \\
				\hline 
			\end{tabular}
			}
		\end{minipage}
		
		%\caption{Meta-atoms for transportation, racing, and sports. The figure shows the atoms that uses them, where atoms/meta-atoms are tagged manually. The table shows the top 4 nearest words and tags for some atoms.}
		%\label{fig:sportmetaatom} 
		\caption{ Meta-atoms for transportation, racing, and sports. The figure shows the atoms that uses them, where atoms/meta-atoms are tagged manually. The table shows the top 4 nearest words and tags for some atoms.}
				\label{fig:metaatom_sports} 
	\end{figure*}


==> linear.tex <==
\section{Linear Structure of Word Senses} \label{sec:linear}

\iffalse 

%of {\em tie},
 % (Please note that the word vectors do not have unit length,  and in fact the theory of of~\newcite{randomdiscourses}  relates their length to the logarithm of the word frequency.)


\iffalse 
We describe a simple experiment that suggests that the embedding for {\em tie} is approximately a weighted sum of the (hypothetical) embeddings of {\em tie1, tie2, ...}. This linear relationship between the embeddings of a word and the embedding of its senses will be the key insight that drives the algorithm design in subsequent sections.  A priori, verifying this conjecture/insight would require tedious hand-labeling of each occurrence of {\em tie} by one of the new tokens {\em tie1}, {\em tie2}, etc, and then training the embeddings for {\em tie1}, {\em tie2}, etc. 

\Tnote{Added several sentences above and below. I think it would be smoother for the readers with these explanation. }
\fi 

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.35\textwidth]{figure/alphabetaVSlogfr-eps-converted-to}
	\caption{Results of creating an artificial polysemous word $w$ by merging two words $w_1$ and $w_2$. The fitted word vector $v_{w}$ for $w$ is found to be very close to $\alpha v_{w_1} + \beta v_{w_2}$ where $v_{w_1}$ and $v_{w_2}$ are the vectors for $w_1$ and $w_2$ respectively.
		The plot shows the coefficients of $\alpha$ and $\beta$ for 100 artificial polysemous words versus the ratio $r$ of the frequencies of $w_1$ and $w_2$ (plotted on a logarithmic scale). }
	\label{fig:alphabetaVSlogfr}
\end{figure}
\setlength{\textfloatsep}{0.1in}
Instead, we  support this proposal by the following experiment: create an artificial polysemous word $w$  by merging random pairs of existing words $w_1$ and $w_2$, so that the ``labeling'' of the two distinct senses in the corpus is known by construction.
%\footnote{We note that this experiment is only meant to verify the linear relationship between the embeddings of the word and its senses, while the real algorithm to decompose polysemous words will come in later sections. } 
%It consists of creating an artificial polysemous word $w$ by combining 
%Concretely, we pick two random (and hence presumably unrelated) words $w_1$ and $w_2$, where $w_1$ is more frequent than $w_2$, and 
Every occurrence of $w_1$ or $w_2$ now counts as an occurrence of $w$. Next, an embedding is computed for $w$ while preserving the embeddings for all other words except $w_1$ and $w_2$, using the objective in~\cite{randomdiscourses} (see equation~\eqref{eqn:PMIobj} in the next subsection), or alternatively, using {\bf GloVe}. 
%\Tnote{added Glove for readers who are not familiar with our paper}

%\Tnote{changed the first sentence in the paragraph below. The old one (commented out) might be a bit confusing. }

Repeating this experiment with various choices of $w_1$ and $w_2$, we found that
indeed $v_{w} \approx \alpha v_{w_1} + \beta v_{w_2}$, where
%Repeating this experiment with a wide range of values for the ratio between the frequencies of $w_1$ and $w_2$, we had the following observations. 
%First, the new vector $v_{w}$ for $w$ always lies close to the subspace spanned by the vectors %$v_{w_1}$ and $v_{w_2}$ for $w_1$ and $w_2$: the 
the average cosine angle between $v_{w}$ and its projection in the subspace spanned by $v_{w_1}$ and $v_{w_2}$ is $0.97$ with standard deviation $0.02$. Some introspection suggests that 
$\alpha$ and $\beta$ must depend upon the ratio $r$ of frequencies of $w_1$ and $w_2$, since their values clearly must change when $r$ goes from $1$ to $\infty$.  (Without loss of generality, assume $w_1$ is more frequent than $w_2$, so $r\geq 1$.)
%  shows how $\alpha, \beta$ depend upon 
%\Tnote{TODO: I understand this sentence is meant to explain the scaling issue Daichi asked. but currently it doesn't seem to be clear what it's talking about given the context} 
%The graph 
Figure~\ref{fig:alphabetaVSlogfr} shows that once $r$ is more than say $3$, then $\alpha \approx 1$ whereas $
  \beta \approx 1- c\log r
$
%\Tnote{TODO -- change to base 10 as Daichi suggested？}
for some constant $c\approx 0.5$. Moreover, the Pearson correlation between $\beta$ and $-\log r$ is $0.67$. (Here and throughout the paper the base of $\log$ is 10.)  %Note this formula is meaningful for sufficiently small $r$, i.e. when $ r < 10^{1/c} \approx 100$. 


%\Tnote{Should specify what is the base of the log. Ideally it should be $e$}

This logarithmic behavior is a good feature, because it allows the less frequent sense to have a larger coefficient, i.e., a sense that accounts for only $\epsilon \ll 1$ fraction of the occurrence of the word can have a coefficient much larger than $\epsilon$ in the linear combination. This makes it not overwhelmed by noise and thus in principle detectable.

\iffalse 
\Tnote{TODO: Now I understand why people don't like the word super-proportionate. I think this might be a rather uncommon word since if some non-native speaker input it into google he/she will fail to find the meaning from the dictionaries supported by google, and there is no good search result explaining the word either. }
\fi 
	\fi 
\subsection{A Mathematical Explanation}
\label{subsec:explanation}

We now give a theoretical explanation of the results of the experiment using the PMI objective of the random walk on discourses model of~\newcite{randomdiscourses}\footnote{Our proof is also adaptible to the related SN objective of~\newcite{randomdiscourses}.}, where the set of word vectors is the solution to the optimization: 
\small
\begin{align}
 \min  \sum_{u, u'}p(u, u')\cdot (\pmi(u,u')- \inner{v_{u}, v_{u'}})^2 \label{eqn:PMIobj}
\end{align}  
\normalsize
where $p(u, u')$ is the empirical probability that words $u$ and $u'$ co-occur within a small distance (say $5$) of each other in the corpus, and $\pmi(u, u') =\log[p(u, u')/(p(u)p(u'))]$. This is reminiscent of the classical PMI method: the inner product of the embeddings has to be matched to the PMI, where the terms have weights given by $p(u, u')$.  

In our experiment, the new artificial word $w$ has co-occurrence probability $p(w,\chi) = p(w_1,\chi)+p(w_2,\chi)$ for every other word $\chi$, and marginal distribution  $p(w)  = p(w_1)+p(w_2)$. The new vector $v_w$ for it is obtained from~\eqref{eqn:PMIobj} using the new co-occurrence probabilities. All the other word vectors remained unchanged, so the optimization reduces to
\small
\begin{align} \label{eqn:zopt}
  v_{w}  =  &~\textup{argmin}_z   f(z), \textup{~where~}  \nonumber\\
  f(z) = &~\sum_{\chi}p(\chi, w) \ (\pmi(\chi,w)- \inner{v_\chi, z})^2. 
\end{align} 
\normalsize
%where $\pmi(\chi,w)$ is defined according to the co-occurrence $p(\chi,w)$ and $p(w)$.

It is impossible to prove anything about the optimum $v_w$ unless we know something else about the co-occurrences $\pmi(\chi, w)$ and the other vectors $v_{\chi}$. We will rely upon some simplifying assumptions, which we justify intuitively; in practice they are only approximately correct, and so are the conclusions derived from them.

%\noindent{\textbf{Simplification 0}:} \emph{Since $w_1$ and $w_2$ are unrelated, assume $p(w_1, w_2) = p(w_1) p(w_2)$.}

\noindent{\textbf{Simplification 1}:} \emph{The original word vectors perfectly fit the PMI model}~\eqref{eqn:PMIobj},\footnote{In general  the argument can be carried through if the fitting has errors which are small and independently chosen from some distribution, say Gaussian.}  \emph{ i.e., every word }$\chi$ \emph{satisfies}  $\pmi(\chi, w_1) = \inner{v_\chi, v_1}$ \emph{and} $\pmi(\chi, w_2) = \inner{v_\chi, v_2}$. 
 
% \noindent{\textbf{Simplification 2}:} \emph{In solving the optimization, restrict attention to words}  $\chi$ \emph{ that co-occur with only one of} $w_1, w_2$ \emph{in the  corpus, not both.}

\noindent{\textbf{Simplification 2}:} \emph{Every word}  $\chi \not\in \{w_1,w_2\}$ \emph{co-occurs with only one of} $w_1$ \emph{and} $w_2$ \emph{, not both.}  

\noindent More precisely, let $T_1$  be the set of words such that $p(\chi,w_1) \neq 0$, and $T_2$ the words such that $p(\chi,w_2) \neq 0$. Since the co-occurrence matrix is sparse, $T_1$ and $T_2$ are two small subsets of the dictionary. Since $w_1$ and $w_2$ are unrelated words that were randomly picked, $T_1 \cap T_2$ is expected to be of negligible size compared to $T_1$ and $T_2$. Formally, if nonzero entries constitute a $p$ fraction of some matrix, then in two randomly picked rows, one expects only $p^2$ fraction of the entries to be nonzero in both. Thus $\chi \in T_1 \cap T_2$ have negligible effect on the optimization and Simplification 2 ignores them.
      
We need a third, somewhat technical simplification; saying, roughly, that the word vectors are distributed fairly uniformly in space. It appears in Section~\ref{sec:explanation} together with the full argument for the following claim. 
			
%There is a third technical simplification that intuitively comes from that the word vectors are distributed fairly uniformly in space, justified in detail in Section~\ref{sec:explanation}.
%To state the simplification, for $i \in \{1,2\}$, denote the mean of the vectors of words that co-occur with $w_i$ as $\mu_i = \sum_{\chi} p(\chi, w_i) v_\chi$, and denote their second moment as $\Sigma_i = \sum_{\chi} p(\chi, w_i) v_\chi v_\chi^\top$.
%
%\noindent{\textbf{Simplification 3}:} \emph{For} $i \in \{1,2\}, \mu_i$ \emph{has the form} $b_i v_{w_i}$ \emph{, and} $\Sigma_i$ \emph{has the form} $\gamma_i v_{w_i} v_{w_i}^\top + \tau_i I,$ \emph{where} $b_i, \gamma_i$ \emph{,and} $\tau_i$ \emph{are scalars.}
%
%We are now ready to state our main claim, whose proof is provided in Section~\ref{sec:explanation}.
%\begin{thm} \label{thm:main}
%Under Simplification 1-3,
%\small
%\begin{align}
	%v_{w} =  \frac{1-\kappa_1c_1}{1+\epsilon_1} v_{w_1} + \frac{1-\kappa_2c_2}{1+\epsilon_2} v_{w_2}  \label{eqn:informal_linearity}
%\end{align}
%\normalsize
%where $c_i$ and $\epsilon_i$ are quantities depending on
%the parameters in the Simplifications and $\|v_{w_i}\|$'s, $\kappa_1 =  \log(1+1/r)$ and $\kappa_2 = \log(1+r)$, and $r = p(w_1) / p(w_2)$.
%\end{thm}

\begin{mainclaim} \label{thm:main}
Under Simplification 1-3,
\small
\begin{align}
	v_{w} \approx (1-\kappa_1c_1) v_{w_1} + (1-\kappa_2c_2)v_{w_2}  \label{eqn:informal_linearity}
\end{align}
\normalsize
where $c_i = O(1)$, $\kappa_1 =  \log(1+1/r)$ and $\kappa_2 = \log(1+r)$ with $r = p(w_1) / p(w_2)$.
\end{mainclaim}
%\Tnote{in the order $-->$ on the order; }
